Human-centric Reward Optimization for Reinforcement Learning-based Automated Driving using Large Language Models

One of the key challenges in current Reinforcement Learning (RL)-based Automated Driving (AD) agents is achieving flexible, precise, and human-like behavior cost-effectively. This paper introduces an innovative approach that uses large language models (LLMs) to intuitively and effectively optimize RL reward functions in a human-centric way. We developed a framework where instructions and dynamic environment descriptions are input into the LLM. The LLM then utilizes this information to assist in generating rewards, thereby steering the behavior of RL agents towards patterns that more closely resemble human driving. The experimental results demonstrate that this approach not only makes RL agents more anthropomorphic but also achieves better performance. Additionally, various strategies for reward-proxy and reward-shaping are investigated, revealing the significant impact of prompt design on shaping an AD vehicle's behavior. These findings offer a promising direction for the development of more advanced, human-like automated driving systems. Our experimental data and source code can be found here

==> Content/CaseStudyStory.tex <==
\section{Case Study: validity of approach} 
\label{sec:casestudy}
\begin{figure*}[h]
\centering
\includegraphics[width=0.9\textwidth]{images/prompt_PREDEF.png}
\caption{Meta Prompt Case Study}
\label{metacase}
\end{figure*}
The following paragraph covers a case study analysis of a random scenario that illustrates the practical capabilities of leveraging the in-context learning ability of LLM in AD highway scenarios. The potential for personalization in highway scenarios by establishing two groups with different meta-prompts is also explored in the following case study.

This section serves to underscore the validity of designed prompts.

In the previous prompt case shown in \ref{metacase}, the scenario can be described as the ego car driving in lane 1 on a highway. There is one vehicle in its current lane. The right lane change is deemed safe by the safety assessment. The previous decision, the ego car made, was to stay idle, which means the ego car is in the process of following the front car. 

This given scenario featured two distinct driving agents, namely the "aggressive" and "conservative" agents, a comprehensive analysis was conducted under controlled conditions.

\begin{figure*}[h]
\centering
\includegraphics[width=0.9\textwidth]{images/prompt_CaseStudy429.jpg}
\caption{Meta Prompt Case Study}
\label{respcase}
\end{figure*}

Each agent's driving behaviour was shaped through a series of user instructions, establishing their respective driving style within the scenario as shown in \ref{respcase}. The scenario itself was meticulously described, incorporating pertinent details to facilitate a thorough understanding of the driving dynamics involved as shown in \ref{metacase}.

Both decisions show strong consistency in humanized behaviour, as well as the conformity of the agent's personalization. 

The agent shows a thorough consideration of the following factors: Safety, Efficiency and Traffic Rules.

For an aggressive agent, the user has stated that efficiency is of higher priority, hence the agent is considering lane right for higher efficiency.

For a conservative agent, the user has stated that safety is of higher priority, hence the agent is considering slowing down to keep distance from the leading car.


Compared with manually designing a reward function, this manner is easier and has demonstrated its effectiveness in guiding the behaviour of an agent. These observations indicate that Large language models (LLMs), like GPT in our case, offer a potential, or even more cost-effective alternative to performing similar roles with human feedback. In certain contexts, LLMs can leverage massive amounts of text data to learn implicitly from human-generated content, interactions, and feedback. 
Introducing LLM significantly reduces the human workload in designing rewards and achieves similar effects. 


% \subsection{Driving Behaviour Analysis}
% \begin{figure}[htbp]
% \centerline{\includegraphics[width=0.9\linewidth]{images/accelerate.png}}
% \caption{Example of decision making align with user object}
% \label{Example}
% \end{figure}
% The above context demonstrates an example of our experiment. In contrast to a conventional RL agent, the agent trained using LLM in conjunction with the RL reward function exhibits driving behaviour that aligns more closely with human intuition. This includes prioritizing safety while maintaining efficiency, minimizing lane changes, and effectively following other vehicles. 


% \begin{figure}[htbp]
%     \centering
%     \begin{subfigure}[b]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{images/CaseStudy1.jpg}
%         \caption{Frame 1}
%         \label{fig:sub1}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{images/CaseStudy2.jpg}
%         \caption{Frame 3}
%         \label{fig:sub2}
%     \end{subfigure}
    
%     \begin{subfigure}[b]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{images/CaseStudy3.jpg}
%         \caption{Frame 5}
%         \label{fig:sub3}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{images/CaseStudy4.jpg}
%         \caption{Frame 7}
%         \label{fig:sub4}
%     \end{subfigure}
%     \caption{Case Study Agent Example}
%     \label{fig:fourfigs}
% \end{figure}


==> Content/Future.tex <==
\section{Future Improvements}

To improve our solution further, we propose:
\begin{itemize}
    \item Enhancing the accuracy of LLM feedback by experimenting with different prompt designs and LLM configurations.
    \item Exploring the impact of LLM-generated feedback on the agent's long-term learning trajectory and its ability to generalize across different tasks and environments.
    \item Exploring incorporating LLM outputs as auxiliary rewards\cite{Adaptive_Reinforcement_Learning_with_LLM-augmented_Reward_Functions} in the learning process of a new reward function in AD scenario.
\end{itemize}

Finally, we anticipate that by employing LLM to reconstruct reward functions, we can tackle some of the more complex transportation scenarios where it is challenging to artificially design reward functions.

By enabling a more nuanced understanding of such situations, LLMs can help improve overall traffic flow. This approach could advance the interaction of automated driving with human drivers dynamically, leading to more efficient and safer transportation systems, by exploring these sophisticated scenarios and refining the interaction between LLM insights and RL agents to address real-world complexities.
